Investigation of reflection-based measurements of microwave kinetic inductance detectors in the optical bands

In this paper, we investigate the single photon response from the reflection of the Microwave Kinetic Inductance Detector (MKID) array. Reflection measurements are carried out using two configurations: one is measured simultaneously with the transmission, and the other is obtained with a single-ended MKID array terminated with an open load. Compared with the transmission, reflection measurements significantly reduce the readout noise of the single-ended MKID array. This is also reflected in the improvement of the median energy resolving power by around 20%-30% under pulsed photon illumination at $\lambda = 405$~nm, mainly due to an increase in the size of the resonance circle on the IQ plane. This method has the potential to be used to read out large MKID arrays.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
